On Galois coverings and tilting modules

Let A be a basic connected finite dimensional algebra over an algebraically closed field, let G be a group, let T be a basic tilting A-module and let B the endomorphism algebra of T. Under a hypothesis on T, we establish a correspondence between the Galois coverings with group G of A and the Galois coverings with group G of B. The hypothesis on T is expressed using the Hasse diagram of basic tilting A-modules and is always verified if A is of finite representation type. Then, we use the above correspondence to prove that A is simply connected if and only if B is simply connected, under the same hypothesis on T. Finally, we prove that if a tilted algebra B of type Q is simply connected, then Q is a tree and the first Hochschild cohomology group of B vanishes

==> s2.1.tex <==
Let us define the $k$-category
$\c End_{\c C}(\bigoplus_{g,i}\ ^g\widehat{T}_i)$ as follows:
\begin{enumerate}
\item[.] the set of objects is $\{\ ^g\widehat{T}_i\ |\ g\in G,\
  i\in\{1,\ldots,n\}\}$ ($^g\widehat{T}_i$ and $^{g'}\widehat{T}_j$
  are considered as different objects if $(i,g)\neq (j,g')$),
\item[.] the space of morphisms from $\,^g\widehat{T}_i$ to
  $\,^h\widehat{T}_j$ is equal to $Hom_{\c
    C}(\,^g\widehat{T}_i,\,^h\widehat{T}_j)$,
\item[.] the composition is induced by the composition of morphisms in
  $MOD(\c C)$.
\end{enumerate}
\begin{rem}
\label{rem2.5}
\begin{enumerate}
\item The $\c C$-modules $\bigoplus_{g,i}\ ^g\widehat{T}_i$ and $F.T$ are
isomorphic.
\item If $G$ is a finite group, then $\c C$ is a finite dimensional
$k$-algebra. In particular, $\c End_{\c C}(\bigoplus_{g,i}\
^g\widehat{T}_i)$ and $End_{\c C}(F.T)$ are isomorphic as $k$-algebras.
\item The $G$-action on $mod(\c C)$ naturally endows $\c End_{\c
C}(\bigoplus_{b,i}\,^g\widehat{T}_i)$ with a structure of free
$G$-category.
\item $\c End_{\c C}(\bigoplus_{i,g}\,^g\widehat{T}_i)$ is a locally
bounded $k$-category if and only if $G_{\widehat{T}_i}=1$ for any
$i$. This is equivalent to say that $F.T$ is a basic $\c C$-module.
\end{enumerate}
\end{rem}
The isomorphisms $\lambda_1,\ldots,\lambda_n$
define the following functor:
\begin{equation}
\begin{array}{cccc}
F_{\widehat{T}_i,\lambda_i}&\c End_{\c C}(\bigoplus_{g,i}\ ^g\widehat{T}_i) & \longrightarrow & End_A(T)\\
&^g\widehat{T}_i&\longmapsto & T_i\\
&^g\widehat{T}_i\xrightarrow{u}\,^h\widehat{T}_j&\longmapsto &
T_i\xrightarrow{\lambda_j\ F_{\lambda}(u)\ \lambda_i^{-1}}T_j
\end{array}\notag
\end{equation}

\begin{lem}
\label{lem2.9}
The functor $F_{\widehat{T}_i,\lambda_i}\colon \c
End(\bigoplus_{i,g}\,^g\widehat{T}_i)\to End_A(T)$ is a Galois covering
with group $G$.
\end{lem}
\noindent{\textbf{Proof:}} For simplicity, we shall write $\c C'$ for $\c
End(\bigoplus_{i,g}\,^g\widehat{T}_i)$ and $F'\colon \c C'\to
End_A(T)$ for $F_{\widehat{T}_i,\lambda_i}$. Recall (see
Remark~\ref{rem2.5}) that $G$ acts freely on $\c E$. Moreover, we have
$F'\circ g=F'$ by construction of $F'$. So, we have a commutative
diagram of $k$-categories and $k$-linear functors:
\begin{equation}
\xymatrix{
\c C'\ar@{->}[d] \ar@{->}[rd]^{F'}&\\
\c C'/G \ar@{->}[r]_{\overline{F'}} & End_A(T)}\tag{$\star$}
\end{equation}
Where $\c C'\to\c E/G$ is the quotient functor.
From the properties verified by
$F_{\lambda}$ (see Section~\ref{section1}) and because
$T_i=F_{\widehat{T}_i,\lambda_i}(^g\widehat{T}_i)$ for any $g,i$, we know
that $F_{\widehat{T}_i,\lambda_i}$ is a covering functor and induces a
surjective mapping $Ob(\c C')\to Ob(End_A(T))$. This implies (see for
example \cite[Prop. 6.1.17]{lemeur_thesis}) that in the diagram
($\star$), the functor $\overline{F'}\colon \c C'/G\to End_A(T)$ is a
covering functor. Finally, $\overline{F'}$ restricts to a bijective
mapping $Ob(\c C')/G=\{\,^g\widehat{T}_i\ |\ g\in G\
i\in\{1,\ldots,n\}\}\to Ob(End_A(T))=\{T_1,\ldots,T_n\}$
so $\overline{F'}$ is an isomorphism. Thus, $F'$ is a Galois
covering with group $G$.\hfill$\square$\\

Since $F_{\widehat{T}_i,\lambda_i}$ is a Galois
covering, it is natural to ask
wether $\c End(\bigoplus_{i,g}\,^g\widehat{T}_i)$ is connected or not. The
following lemma partially answers this question.
\begin{lem}
\label{lem2.8}
If $\c C$ is not connected, then $\c End_{\c
    C}(\bigoplus_{i,g}\,^g\widehat{T}_i)$ is not connected.
\end{lem}
\noindent{\textbf{Proof}:} 
For simplicity let us set $\c E:=\c End_{\c
  C}(\bigoplus_{i,g}\,^g\widehat{T}_i)$. Assume that $\c C$ is not
connected and let $\c
C=\coprod_{x\in I}\c C_x$ where the $\c C_x$'s are the connected
components of $\c C$. Let $i\in\{1,\ldots,n\}$, since
$\widehat{T}_i\in ind(\c C)$, there exists a unique $x_i\in I$ such
that $\widehat{T}_i\in ind(\c C_{x_i})$. Let us set:
\begin{equation}
G_{x_0}=\{g\in G\ |\ g(\c C_{x_0})=\c C_{x_0}\}\notag
\end{equation}
Since $G$ acts transitively on $\{\c C_{x}\ |\ x\in I\}$, for every
$i\in\{1,\ldots,n\}$ there exists $g_i\in G$ such that $g_i(\c
C_{x_0})=\c C_{x_i}$ (in particular $g_1\in G_{x_0}$).
Therefore:
\begin{equation}
(\forall i\in\{1,\ldots,n\})\ \ ^{g_i^{-1}}\widehat{T}_i\in mod(\c
C_{x_0})\notag
\end{equation}
Let us set $O$ to be the following set of objects of $\c E$:
\begin{equation}
O:=\{\,^g\widehat{T}_i\ |\ i\in\{1,\ldots,n\}\ \text{and}\ gg_i\in
G_{x_0}\}\subseteq Ob(\c E)\notag
\end{equation}
Remark that $O$ satisfies the following:
\begin{enumerate}
\item[.] $O\neq\emptyset$ for $\widehat{T}_1\in O$.
\item[.] Since $\c C$
is not connected and since $G$ acts
transitively on $\{\c C_x\ |\ x\in I\}$ we have $G_{x_0}\subsetneq G$.
Let $g\in G\backslash G_{x_0}$, then $gg_1\not\in G_{x_0}$
(recall that $g_1\in G_{x_0}$) and $^g\widehat{T}_1\not\in O$. Hence
$O\subsetneq Ob(\c C)$.
\item[.] For any $^g\widehat{T}_i\in Ob(\c E)$, we have
  $^g\widehat{T}_i\in O$ if and only if $^g\widehat{T}_i\in ind(\c
  C_{x_0})$. As a consequence, there is no non zero morphism in $\c E$
  between an object in $O$ and an object in $Ob(\c E)\backslash O$.
\end{enumerate}
These three facts prove that $\c E$ is not connected.\hfill$\square$\\

==> s7.tex <==
Throughout this section, $A'$ will be a basic finite dimensional 
 $k$-algebra and $F\colon A'\to A$ will be a Galois covering
with (finite) group $G$. The aim of this section is to compare the
posets $\c T_A$ and $\c T_{A'}$. In this purpose, we begin with the
following proposition:
\begin{prop}
\label{prop3.1}
Let $T\in\c T_A$, then $F.T\in \c T_{A'}$. Moreover $T$ is of the
first kind w.r.t. $F$. Finally, if $X$ is an indecomposable summand of
$T$ and if $\widehat{T}\in mod(A')$ verifies
$F_{\lambda}(\widehat{X})\simeq X$ then $G_{\widehat{X}}=1$.
\end{prop}
\noindent{\textbf{Proof:}}  From Lemma~\ref{lem1.1} applied to $T$, we have
$pd_{A'}(F.T)<\infty$ together with:
\begin{equation}
(\forall i\geqslant 1)\ \ Ext_{A'}^i(F.T,F.T)\simeq
Ext_A^i(F_{\lambda}F.T,T)\simeq Ext_A^i(\bigoplus_{g\in G}T,T)\simeq
\bigoplus_{g\in G}Ext_A^i(T,T)=0\notag
\end{equation}
Thus $F.T$ is an exceptionnal $A'$-module. Moreover, we have an exact
sequence in $mod(A)$:
\begin{equation}
0\to A\to T_1\to\ldots\to T_r\to 0\notag
\end{equation}
where $T_i\in add(T)$ for every $i$. Applying $F.$ to this exact
sequence gives an exact sequence in $mod(A')$:
\begin{equation}
0\to F.A\simeq A'\to F.T_1\to\ldots\to F.T_r\to 0\notag
\end{equation}
where $F.T_i\in add(F.T)$ for every $i$. Hence $F.T$ is a tilting $A'$-module.

Now let us prove that $F.T$ is basic and that $T\in mod_1(A)$. Since
$T\in \c T_A$, we
have $T=T_1\bigoplus\ldots\bigoplus T_n$ with $T_i\in ind(A)$ for each $i$
and $T_i\not\simeq T_j$ if $i\neq j$. For each $i$, let us write
$F.T_i=\bigoplus_{l=1}^{m_i}X_{i,l}$ with $X_{i,l}\in ind(A')$. Hence
$F.T=\bigoplus_{l,i}X_{i,l}$ is a tilting $A'$-module and is the direct
sum of $\sum_{i=1}^n m_i$ indecomposable $A'$-modules, so (see
\cite[Thm 1.19]{miya}):
\begin{equation}
\sum\limits_{i=1}^nm_i\geqslant rk\,K_0(A')=n.|G|\tag{$i$}
\end{equation}
Moreover, we have for each $i$:
\begin{equation}
\bigoplus\limits_{g\in
  G}T_i=F_{\lambda}F.(T_i)=\bigoplus\limits_{l=1}^{m_i}F_{\lambda}(X_{i,l})\tag{$ii$}
\end{equation}
where the last term (resp. the first term) of the equality is the
direct sum of at least $m_i$ (resp. exactly $|G|$) indecomposable
$A$-modules, so:
\begin{equation}
(\forall i\in\{1,\ldots,n\})\ \ |G|\geqslant m_i\tag{$iii$}
\end{equation}
From $(i),(ii)$ and $(iii)$ we deduce that:
\begin{enumerate}
\item[$(iv)$] $m_i=|G|$ for each $i$,
\item[$(v)$] $F_{\lambda}(X_{i,l})\simeq T_i$ for each $i,l$ (in
  particular, for any $i$, $T_i$ is of the first kind w.r.t. $F$),
\end{enumerate}
Hence $F.T=\bigoplus_{l,i}X_{i,l}$ is a tilting $A'$-module and is the
direct sum of $\sum_im_i=n.|G|=rk\,K_0(A')$ indecomposable
$A'$-modules. This shows that (see \cite[Thm 1.19]{miya}) $F.T$ is basic (and
therefore $F.T\in\c T_{A'}$), and $(v)$ shows that $T\in mod_1(A)$.

Finally, let $X\in ind(A)$ be a direct summand of $T$ and let
$\widehat{X}\in ind(A')$ verify $F_{\lambda}(\widehat{X})\simeq
X$. Thus, we have $F.(X)\simeq \bigoplus_{g\in
  G}\,^g\widehat{X}$. Moreover, $F.X$ is a direct summand of $F.T$
which is basic. So $\bigoplus_{g\in G}\,^g\widehat{X}$ is basic,
i.e. $G_{\widehat{X}}=1$.\hfill$\square$\\

\begin{rem}
\label{rem3.2}
. Proposition~\ref{prop3.1} proves that $F.$ sends tilting $A$-modules
to tilting $A'$-modules.\\
. In general, given $X\in ind(A')$ (with $G$ non necessarily finite),
the property $G_{X}=1$ (like in
Proposition~\ref{prop3.1}) implies that $F_{\lambda}(X)$ is
indecomposable (see \cite[3.5]{gabriel}).
\end{rem}

The following example shows that $F_{\lambda}$ does not always
preserve tilting modules.
\begin{ex}
\label{ex3.3}
Let $A$ be the path algebra of the quiver $Q$ equal to:
\begin{equation}
\xymatrix{
&2\ar@{->}[rd]&\\
1\ar@{->}[ru]\ar@{->}[rr]&&3
}\notag
\end{equation}
Let $A'$ be the path algebra of the quiver $Q'$ equal to:
\begin{equation}
\xymatrix{
&1\ar@{->}[ld]\ar@{->}[r]&3'&\\
2\ar@{->}[rd]&&&2'\ar@{->}[lu]\\
& 3& 1'\ar@{->}[l]\ar@{->}[ru]
}\notag
\end{equation}
The mapping $i,i'\mapsto i$ ($i\in\{1,2,3\}$) uniquely defines a
Galois covering $A'\to A$ with group $\mathbb{Z}/2\mathbb{Z}$. For $x$
a vertex of $Q$ or $Q'$, let $P_x$ be the associated indecomposable
projective module and let $\tau_A$ (resp. $\tau_{A'}$) be the
Auslander-Reiten translation (see \cite{ars}) of $A$ (resp. of $A'$).
Let $T=P_1\bigoplus P_2\bigoplus P_3\bigoplus P_{1'}\bigoplus
P_{2'}\bigoplus\tau_{A'}^{-1}(P_{3'})$ be the APR-tilting $A'$-module
associated with the sink $3'$ of $Q'$ (see \cite{apr}). Then:
\begin{enumerate}
\item[.] $P_3\bigoplus\tau_{A'}^{-1}(P_{3'})$ is a selforthogonal
  $A'$-module.
\item[.]
  $F_{\lambda}(P_3\bigoplus\tau_{A'}^{-1}(P_{3'}))=P_3\bigoplus\tau_A^{-1}(P_3)$ is not selforthogonal
 because of the almost split sequence in $mod(A)$:
\begin{equation}
0\to P_3\to P_1\bigoplus P_2\to\tau_A^{-1}(P_3)\to 0\notag
\end{equation}
\end{enumerate}
This shows that $F_{\lambda}(T)$ is not selforthogonal and therefore not tilting.
\end{ex}

Although $F_{\lambda}$ does not always transform a tilting $A'$-module
into a tilting $A$-module, it is possible to characterise those tilting
$A'$-modules $T$ such that $F_{\lambda}(T)$ is tilting. We establish
this characterisation in the following proposition.
\begin{prop}
\label{prop3.4}
$1)$ If $T\in\c T_A$ then $G_{F.T}=G$.\\
$2)$ Let $X\in \c T_{A'}$ verify $G_X=G$. Let $T\in mod(A)$ be a basic
$A$-module such that $add(T)=add(F.X)$. Then $T\in \c T_A$ and
$X\simeq F.T$.\\
$3)$ Let $X\in\c T_{A'}$, then $F_{\lambda}(X)$ is tilting if and only
if $G_X=G$.
\end{prop}
\noindent{\textbf{Proof:}} $1)$ is a consequence of the definition of
$F.$. Let us prove $2)$. From Lemma~\ref{lem1.1} we get
$pd_A(F_{\lambda}(X))\leqslant pd_A(T)<\infty$. Since $X$ is selforthogonal and
$G$ is finite, Lemma~\ref{lem1.1} implies that:
\begin{equation}
(\forall i\geqslant 1)\ \ Ext_A^i(F_{\lambda}(X),F_{\lambda}(X))\simeq
Ext_{A'}^i(X,F.F_{\lambda}(X))\simeq
Ext_{A'}^i(X,\bigoplus\limits_{g\in G}\,^gX)\simeq
\bigoplus\limits_{g\in G}Ext_{A'}^i(X,\,^gX)=0\notag
\end{equation}
So $F_{\lambda}(X)$ and $T$ are selforthogonal. This shows that $T$
is an exceptionnal and basic $A$-module. Hence, in order to prove that
$T\in\c T_A$, it suffices to prove that $d(T)\geqslant n$ (see
\cite[Thm 1.19]{miya}, recall that $d(T)$ is the number of
indecomposables whose direct sum is $T$). The equalities $add(T)=add(F_{\lambda}(X))$ and $G_X=G$
imply that:
\begin{equation}
add(F.T)=add(F.F_{\lambda}(X))=add(\bigoplus\limits_{g\in G}\,^gX)=add(X)\tag{$i$}
\end{equation}
Since $X$ is basic, we infer that $X$ is a direct summand of
$F.T$. In particular, we have:
\begin{equation}
d(F.T)\geqslant d(X)=n.|G|\tag{$ii$}
\end{equation}
the last equatity of $(ii)$ is due to the fact that $X\in\c
T_{A'}$. Using $(ii)$ we get:
\begin{equation}
d(T)=\frac{1}{|G|}d(\bigoplus\limits_{g\in
  G}T)=\frac{1}{|G|}d(F_{\lambda}F.(T)) \geqslant \frac{1}{|G|}
d(F.T)\geqslant \frac{1}{|G|} n|G|=n\notag
\end{equation}
Hence $T$ is an exceptionnal basic $A$-module satisfying
$d(T)\geqslant n$. So $T\in\c T_A$ and $d(T)=n$. Now let us prove that
$F.T\simeq X$. From Proposition~\ref{prop3.1} we know that $F.T$ is
basic. Since $X$ is basic as well and since $add(X)=add(F.T)$ (see
$(i)$ above) we infer that $X\simeq F.T$. This proves $2)$.

Let us prove $3)$. If $G_X=G$, then $add(F_{\lambda}(X))=add(T)$ with
$T\in \c T_A$ (see $2)$), so $F_{\lambda}(X)$ is tilting. Conversely,
suppose that $F_{\lambda}(X)$ is tilting. Then we get from
Lemma~\ref{lem1.1} (recall that $G$ is finite):
\begin{equation}
(\forall i\geqslant 1)\ \
0=Ext_A^i(F_{\lambda}(X),F_{\lambda}(X))\simeq
Ext_{A'}^i(X,F.F_{\lambda}(X))\simeq \bigoplus\limits_{g\in G}Ext_{A'}^i(X,\,^gX)\notag
\end{equation}
So:
\begin{equation}
(\forall i\geqslant 1)\ (\forall g\in G)\left\{
\begin{array}{l}
Ext_{A'}^i(X,\,^gX)=0\\
Ext_{A'}^i(\,^gX,X)\simeq Ext_{A'}^i(X,\,^{g^{-1}}X)=0
\end{array}\right.\notag
\end{equation}
Since $^gX\in\c T_{A'}$ for any $g\in G$ we infer that $^gX\simeq X$
for any $g\in G$.\hfill$\square$\\

Before stating the theorem comparing $\c T_A$ and $\c T_{A'}$, we
remark that the action of $G$ on $mod(A')$ naturally defines an action
on the poset $\c T_{A'}$ (the action is compatible with the order:
$X\geqslant X'\Rightarrow \,^gX\geqslant \,^gX'$).
\begin{thm}
\label{thm3.5}
The mapping:
\begin{equation}
\begin{array}{rrcl}
\iota\colon & \c T_A & \longrightarrow & \c T_{A'}\\
& T& \longmapsto & F.T
\end{array}\notag
\end{equation}
is a well defined injective morphism of posets. It's image is equal
to:
\begin{equation}
\c T_{A'}^G=\{T\in\c T_{A'}\ |\ (\forall g\in G)\ \,^gX\simeq X\}\notag
\end{equation}
\end{thm}
\noindent{\textbf{Proof:}} Thanks to Proposition~\ref{prop3.1} and
Proposition~\ref{prop3.4} we only need to prove that $\iota$ is
injective and increasing. If $T,T'\in\c T_{A'}$ are such that $F.T\simeq F.T'$
then $\bigoplus_{g\in G} T\simeq F_{\lambda}F.(T)\simeq
F_{\lambda}F.(T')\simeq \bigoplus_{g\in G} T'$ and therefore $T\simeq
T'$ (recall that $T$ and $T'$ are basic). So $\iota$ is
injective. Now assume that $T\leqslant T'$ in $\c T_A$. Let $X\in
(F.T)^{\perp}$, then Lemma~\ref{lem1.1} implies that:
\begin{equation}
(\forall i\geqslant 1)\ \ 0=Ext_{A'}^i(F.T,X)\simeq Ext_A^i(T,F_{\lambda}(X))\notag
\end{equation}
So $F_{\lambda}(X)\in T^{\perp}\subseteq T'^{\perp}$. Using once more
Lemma~\ref{lem1.1} we infer that:
\begin{equation}
(\forall i\geqslant 1) \ \ 0=Ext_A^i(T',F_{\lambda}(X))\simeq Ext_{A'}^i(F.T',X)\notag
\end{equation}
So $X\in (F.T')^{\perp}$. This shows that $\iota$ is a morphism of
posets.\hfill$\square$\\

In Proposition~\ref{prop3.1} we have proved that any basic tilting
$A$-module is of the first kind w.r.t. $F$. Therefore,
Definition~\ref{def2.4} and Remark~\ref{rem2.5} give a Galois covering
$F_T\colon End_{A'}(F.T)\to End_A(T)$ with group $G$. In view of the
proof of Theorem~\ref{thm0.1} we now
verify that this Galois covering is connected.
\begin{prop}
\label{prop3.6}
Let $T$ be a basic tilting $A$-module. Then
the Galois covering $F_T\colon End_{A'}(F.T)\to End_A(T)$  is connected.
\end{prop}
\noindent{\textbf{Proof:}} Let us write $T=T_1\bigoplus\ldots\bigoplus
T_n$ (with $T_i\in ind(A)$). For each $i$ let us fix $\widehat{T}_i\in
ind(A')$ verifying $F_{\lambda}(\widehat{T}_i)\simeq T_i$. In order to
prove that the Galois covering $F_T$ is connected we thus
need to prove that the $k$-category $End_{A'}(\bigoplus_{g\in
  G}\,^g\widehat{T}_i)$  is locally bounded
and connected. From Proposition~\ref{prop3.1} we know that $F.T\simeq
\bigoplus_{g\in
  G}\,^g\widehat{T}_i$ is a basic tilting $A'$-module. So $End_{A'}(\bigoplus_{g\in
  G}\,^g\widehat{T}_i)$ is a finite dimensional basic and connected $k$-algebra,
i.e. a locally bounded and connected.\hfill$\square$\\
